On Enhancing Root Cause Analysis with SQL Summaries for Failures in Database Workload Replays at SAP HANA

Capturing the workload of a database and replaying this workload for a new version of the database can be an effective approach for regression testing. However, false positive errors caused by many factors such as data privacy limitations, time dependency or non-determinism in multi-threaded environment can negatively impact the effectiveness. Therefore, we employ a machine learning based framework to automate the root cause analysis of failures found during replays. However, handling unseen novel issues not found in the training data is one general challenge of machine learning approaches with respect to generalizability of the learned model. We describe how we continue to address this challenge for more robust long-term solutions. From our experience, retraining with new failures is inadequate due to features overlapping across distinct root causes. Hence, we leverage a large language model (LLM) to analyze failed SQL statements and extract concise failure summaries as an additional feature to enhance the classification process. Our experiments show the F1-Macro score improved by 4.77% for our data. We consider our approach beneficial for providing end users with additional information to gain more insights into the found issues and to improve the assessment of the replay results.

==> notes.tex <==
\begin{itemize}
    \item Root causes for creating context
    \item What is the color status of the replays -- colors across the times we have rated replays - Does that warrant context?
    \item What is the current performance of the model
    \item Can we show the performance change - by grouping across the parent reason concept? - should we present this as an intermediate concept? And say this is still not enough?
    \item how do we position this as extension of mira?
\end{itemize}


\begin{itemize}
    \item distance between the two different reasons - change  - increase in distance by 20% ... x'/X
    \item 
    \item 
    \item how many items get deduplicated by adding context
    \item 
\end{itemize}



Towards Contextualizing Workload Replay Failures with SQL Summary for Root Cause Analysis at SAP HANA


Towards Contextualizing Workload Replay Failures with SQL Summary for Root Cause Analysis at SAP HANA

Towards 
Contextualizing Workload Replay Failures
with SQL Summaries
for enhancing Root Cause Analysis at SAP HANA


Towards enhancing Root Cause Analysis for failures in Database Workloads Replays
with SQL Summaries
 at SAP HANA


On Enhancing Root Cause Analysis with SQL Summaries for Failures in Database Workload Replays at SAP HANA
On Enhancing Root Cause Analysis with SQL Summaries for Failures while Replaying Database Workloads at SAP HANA



Bad:
On Enhancing Root Cause Analysis with SQL Summaries for Replay Failures in Database Workloads at SAP HANA

==> related_work.tex <==

% \textit{SQL Workload Summarization}: Numerous works focus on developing effective representations for SQL queries using natural language processing techniques in order to model various aspects of databases. \cite{tang2021forecasting} at Twitter have made use of a TFIDF-based representation of SQL statements for the purpose of forecasting query costs. \cite{jain2018query2vec} introduce Query2vec, a technique for learning vectorized representations of SQL queries from database workloads and execution plans. They employ this technique to summarize database workloads and to identify query patterns that result in runtime errors. \cite{li2019detection} introduced improved TFIDF for vectorizing the SQL queries for the purpose detecting SQL injections attacks.  \cite{zahir2016recommendation} recommend existing execution plans based on similarities of the vectorized SQL queries and execution plans. We attempt to learn representations for the SQL statement strings using TFIDF \cite{salton1986introduction} and Doc2Vec~\cite{le2014distributed} in order to use them in our framework for automatically classifying failures during replay.

% \textit{LLMs for SQL summarization}: Captured workloads contain SQL statements of which several might be order dependent. In replay based testing, the workload is run as captured without any modifications to the parameters, dynamic variables etc. This might lead to failure -- ALL REPETITION




==> reviews_FSE.tex <==

FSE 2024 HotCRP <noreply-fse2024-industry@hotcrp.com>


Dear authors,

We regret to inform you that your submission entitled “ On Enhancing
Root Cause Analysis with SQL Summaries for Failures in Database Workload
Replays at SAP HANA” has not been accepted to the ESEC/FSE 2024 industry
track.

The competition was strong. This year, the ESEC/FSE we received more
than 100 submissions. Each paper was reviewed by at least three program
committee members and extensively discussed online.
Acceptance/rejection decisions were based only on the assessed quality
of the submission.

We understand that this news may be disappointing, and we appreciate the
significant effort involved in preparing and submitting your paper.

Below, we have enclosed the reviews of your paper. We hope that they
will help you to revise the paper for a successful future resubmission.

Review #39A
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper describes a process for lowering the amount of false positives when analyzing errors after rerunning recorded queries in a large database setting, The process builds on a supervised machine learning method to detect the root causes of these errors. As an enhancement a Large Language Model is used to create summaries of SQL statements and error messages, which improves the classification and training process with about 2%.

Comments for authors
--------------------
The paper is well written and contains innovative use of machine learning techniques. The results are quantitatively evaluated. There are two major concerns with the paper: 1) it is not clear what the industrial context is. We know that the DBMS is SAP HANA, but nothing more. Just two sentences would remedy this. 2) Very little is written about the motivation of the choice of technologies, methods and metrics. For instance, why is KNN used, why is a 5-fold  cross validation used?

Solution:
Add refs of why 5 CV -- that 5 cv is standard



* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #39B
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
When replaying the database workload, handling unseen novel issues not found in the training data is one general challenge of machine learning approaches with respect to generalizability of the learned model. Authors find that retraining with new failures is inadequate due to features overlapping across distinct root causes. Thus, authors take advantage of a large language model (LLM) to analyze failed SQL statements and extract concise failure summaries as an additional feature to enhance the classification process. The experiments show the F1-Macro score improved by 2% for our data.

Comments for authors
--------------------
1. Strengths
+ The usage of ChatGPT to address existing problems is a hot topic and the scenario described in the paper is a good fit.
+ The authors introduce the background well which shows the importance of addressing the problem.

2. Weaknesses
- The evaluation experiments didn’t include the statistical significance tests.
- The evaluation results show that the improvement is tiny, which raises concerns about the practicality of the strategy.
- The strategy mainly relies on ChatGPT which limits the novelty.

3. Comments for authors

3.1 Significance

i. The paper didn’t discuss much about the statistical significance of the experiment outcome.

ii. Given the fact that the performance is only promoted in a very tiny way, I think the authors may want to conduct more experiments to show the practicality of the strategy.

3.2 Soundness

i. The paper compares one other algorithm that could also be used to summarize the statements with ChatGPT. However, the outcome is not introduced in a detailed way and authors may want to add more algorithms for comparison.

ii. Using the ChatGPT may bring the concern of security which authors may want to discuss in the paper.

iii. The paper doesn’t discuss the flaky tests which may influence the outcome of the experiments.

iv. Authors may also want to introduce the effect size of the features after the adoption of ChatGPT.

3.3 Novelty

i. Authors take advantage of ChatGPT to summarize the statements which may limit the novelty of the paper.

3.4 Presentation

i. The writing of the paper is generally good and easy to follow.

ii. Authors may want to add a related work section to compare their work with existing research.

3.5 Verifiability

i. The paper doesn’t discuss much about its verfiability and the replication package is not provided.

3.6 Some minor comments

i. Authors may want to move the sentence in the Introduction section of explaining the importance of replaying recorded databases with citations to the beginning of the paragraph.

ii. There is some other existing research about the usage of ChatGPT to summarize the text. Authors may want to compare them in the related work section.


iii. This sentence is hard to understand: ”providing an end users additional information”


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #39C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper is about enhancing root cause analysis (RCA) for failures in replying database workloads at SAP HANA. A machine-learning based RCA system called MIRA has been used in production for years but the quality (F1-score) degraded recently due new failure types that require additional information to the training data. This, however, requires thorough evaluation before production ramp up that takes time. The approach constructs a new feature by utilizing a LLM analyzing a sequence of failed SQL statements to extract failure summaries.

Comments for authors
--------------------
Page 1:

I am not sure what are classified as failures during replays. For example, do you validate for matching query results? Also, what are considered false positives?

"This can result in up to 1 million failures per replay" =>
- I don't see the claim in the paper being referenced.
- The absolute number does not really show how bad the failures are. It is better to show the percentage.

Section 2.1, Figure 3 mentioned here but is put at Page 4, making the reader hard to follow.

Summary:
- It is not clear about the intuition why a SQL summary generated on a failed event improves MIRA.
- As shown in Section 4, it looks to me the improvement is not significant (2% for F1-macro decline in accuracy)

solution:
Does this 2\% mean too much effort, for just 2\%  --- tradeoff is not enough!
JUSTIFY

in regression  -- 2\% is significant ... increases the F1 score  
include the  


---------------------------------------------------------

If you have any questions or comments, please do not hesitate to contact
us.

Best wishes,
Roshanak Zilouchian Moghaddam and Jan Bosch
ESEC/FSE 2024 Industry Track Chairs


